Average-reward model-free reinforcement learning: a systematic review and literature mapping

Reinforcement learning is important part of artificial intelligence. In this paper, we review model-free reinforcement learning that utilizes the average reward optimality criterion in the infinite horizon setting. Motivated by the solo survey by Mahadevan (1996a), we provide an updated review of work in this area and extend it to cover policy-iteration and function approximation methods (in addition to the value-iteration and tabular counterparts). We present a comprehensive literature mapping. We also identify and discuss opportunities for future work.

==> support_algo.tex <==
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{xcolor}
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{black}{#1}}
\SetCommentSty{mycommfont}
\SetKwInput{KwInput}{Input}                %
\SetKwInput{KwOutput}{Output}              %

\SetKw{Andd}{and} %
\SetKw{Break}{break}
\SetKw{Continue}{continue}
\SetKw{Return}{return}


==> support_linking.tex <==
\usepackage{url}            %

\usepackage[hidelinks, bookmarksnumbered]{hyperref}

\hypersetup{
  colorlinks   = true,
  urlcolor     = blue,
  linkcolor    = blue,
  citecolor   = blue
}

